Transient Evaluation of Non-Markovian Models by Stochastic State Classes and Simulation

Non-Markovian models have great expressive power, at the cost of complex analysis of the stochastic process. The method of Stochastic State Classes (SSCs) derives closed-form analytical expressions for the joint Probability Density Functions (PDFs) of the active timers with marginal expolynomial PDF, though being hindered by the number of concurrent non-exponential timers and of discrete events between regenerations. Simulation is an alternative capable of handling the large class of PDFs samplable via inverse transform, which however suffers from rare events. We combine these approaches to analyze time-bounded transient properties of non-Markovian models. We enumerate SSCs near the root of the state-space tree and then rely on simulation to reach the target, affording transient evaluation of models for which the method of SSCs is not viable while reducing computational time and variance of the estimator of transient probabilities with respect to simulation. Promising results are observed in the estimation of rare event probabilities.

==> 02-sscs-old.tex <==
\section{Background}

\subsection{Different Types of Petri Nets}
In the theoretical modeling and analysis of complex systems, it is handy to have an elaborate modeling mechanism that is applicable to a wide range of systems.
One of the most famous ones is the so-called \ac{PN}~\cite{petri-nets}, where the current state of a system is described by the occupation of \emph{places} with \emph{tokens} and possible changes are specified by \emph{transitions}.
One of the primary goals in \ac{PN} analysis is to detect which different allocations of places are possible at all, ignoring the time completely.

In the analysis conducted in our experiments, however, we are interested in the time behavior of the transitions. This can be formalized in extended versions of \acp{PN}, where we will focus on two of them.
The first one is the \ac{TPN} where we associate each transition with the earliest time and the latest time where it can fire~\cite{tpn-analysis}:

\begin{definition}[\Acl{TPN}]
	A \ac{TPN} is a tuple $\splitatcommas{\langle P, T, A^{-}, A^{+}, A^{\bullet}, m_0, EFT, LFT\rangle}$, where the individual components are defined as follows:
	\begin{itemize}
		\item $P$ set of places, $T$ set of transitions
		\item $A^{-} \in P\times T$, $A^{+} \in T\times P$, $A^{\bullet} \in P\times T$ are the sets of preconditions, postconditions, and inhibitor arcs.
		\item $m_0 \in \mathbb{N}^P$ initial marking
		% \item Update function $U(t) : \mathbb{N}^P \rightarrow \mathbb{N}^P$, associates for each transition $t$ an old marking with a new one.
		\item $EFT : T \rightarrow \mathbb{Q}_{\geq 0}$ and $LFT : T \rightarrow \mathbb{Q}_{\geq 0} \cup \{\infty\}$ defining for each transition the earliest and latest time to fire. When it holds $EFT(t) = LFT(t)$ for a transition $t$, we refer to it as a deterministic transition, when additionally $EFT(t) = 0$ and $LFT(t) = 0$ holds, the transition is called immediate. %{\color{red}(Why set $\mathbb{Q}$ and not $\mathbb{R}$?)}
	\end{itemize}
\end{definition}

One goal of a \ac{TPN} is to find out which sequences of transition firings are possible, not at which probability they happen. If we want to associate certain transitions with a probabilistic time behavior, we make use of an \ac{STPN}~\cite{stochastic-state-classes}:
\begin{definition}[\Acl{STPN}]
	An \ac{STPN} is a tuple $\splitatcommas{\langle P, T, A^{-}, A^{+}, A^{\bullet}, m_0, EFT, LFT, F, W\rangle}$, where we refer for $P$, $T$, $A^{-}$, $A^{+}$, $A^{\bullet}$, $m_0$, $EFT$, and $LFT$ to the definition of a \ac{TPN} and all other components are defined as follows:
	\begin{itemize}
		\item $F(t)$ is the \ac{CDF} for each transition over the domain $\splitatcommas{[EFT(t), LFT(t)]}$.
		\item $W : T \rightarrow \mathbb{R}_{>0}$ assigns each transition with a weight.
	\end{itemize}
\end{definition}

As can be seen, the \ac{STPN} extends the \ac{TPN} by adding to each transition a \ac{CDF} denoting its probabilistic time behavior as well a weight value being used if two transitions are in competition.
The weight is used to randomly decide between multiple transitions. Additionally, we could add a priority to each transition which can be used to strictly favor one transition over another.
The reason why we introduced \acp{TPN} alongside \acp{STPN} is that we utilize both during this work since the state space of a \ac{TPN} can be easier analyzed than for an \ac{STPN}. We can gain information out of a \ac{TPN} at a low cost and resort to analysis outcomes of the \ac{TPN} for the \ac{STPN} analysis itself. This property can serve as basis for determining a heuristic for the developed approach, as discussed in Section~\ref{sec:automated-splitting-techniques} and Section~\ref{sec:exploiting-rareness}.

It is worth mentioning that the \ac{STPN} is a generalization of other \ac{PN} models which involve probabilistic time behavior.
One popular example is the \ac{GSPN} which features only exponential and immediate transitions~\cite{gspn-paper}.
The restriction to exponential transitions is a huge benefit as the exponential distribution features the memoryless property, whereas we can ignore the elapsed time to some extent and model the state-space by a \ac{CTMC}. Furthermore, the \ac{CTMC} can be discretized into a \ac{DTMC} allowing further analysis with techniques like \emph{uniformization}~\cite{uniformization-algorithm}.
Since our aim is to analyze systems without the Markovian properties, we do not focus on these in this work.

With \acp{SSC}, \acp{SC} are extended by adding a \ac{JPD} defined over the domain of an \ac{SC}. As a consequence, an \ac{SSC} does not only describe which timings are possible but also, how likely they are. Formally, \acp{SSC} can be defined as follows~\cite{stochastic-state-classes}:
\begin{definition}[\Acl{SSC}]
	An \ac{SSC} is a tuple $\Sigma = \langle m, D, f_\tau(x)\rangle$, where $m$ represents the marking of the current state, $D$ the domain (e.g., the parts of $f_\tau(x)$ with non-zero probability), and $f_\tau(x)$ the \ac{JPD} of the \acp{RV} describing the next firing times to a new transition.
\end{definition}

It is important to store the \ac{JPD} of the involved timings and not only the marginal distributions since the firings are not necessarily stochastically independent.

\subsection{State Classes and Stochastic State Classes}
{\color{red}Find appropriate introduction here}

In mathematical terms, an \ac{SC} can be defined as follows:
\begin{definition}[\Acl{SC}]
	An \ac{SC} is a pair $\langle m, D\rangle$ where $m$ is a marking and $D$ is a firing domain for the transitions $t_i$ with $i \in \{1, ..., n\}$ and $n$ being the number of active transitions. The domain $D$ is described with inequalities of the form
	\begin{align*}
		D = \begin{cases}
			\tau(t_i) - \tau(t_j) \leq b_{i,j} & \forall i, j \in \{1, ..., n\}, i\neq j\\
			b_{*,i} \leq \tau(t_i) \leq b_{i,*} & \forall i \in \{1, ..., n\}
		\end{cases}
	\end{align*}
	where $b_{i, j} \in \mathbb{R} \cup \{\infty\}$ with $i, j \in \{1, 2, ..., n\} \cup \{*\}$.
%	When $i=*\vee j=*$ holds, $b_{i, j}$ has to be non-negative.
\end{definition}
The inequality system of an \ac{SC} is defined by bounding the difference between the firing times of two transitions as well as the firing time of a transition individually. When treating $t_*$ as an artificial transition for which we set $\tau(t_*) = 0$, it becomes apparent that all inequalities can be represented in the form:
\begin{align}
	\tau(t_i) - \tau(t_j) \leq b_{i, j} \qquad \forall i, j \in \{1, ..., n\} \cup \{*\}, i\neq j
\end{align}
Utilizing this form, the \ac{SC} can be efficiently stored in a \ac{DBM}.
Furthermore, it can be shown that an \ac{SC} is uniquely represented as a \ac{DBM} when the variables are sorted and the \emph{triangular inequality} with
\begin{align}
	b_{i, j} \leq b_{i, h} + b_{h, j} \qquad \forall i, h, j \in \{1, ..., n\} \cup \{*\}, i\neq h\neq j
\end{align}
holds.
As a consequence, when interpreting the matrix as a weighted graph, we can define an all-pair shortest path problem for deriving a so-called \emph{normal} form and calculate the shortest distance between each node with the help of, e.g., the \ac{FW} algorithm~\cite{cormen01algorithms,rosen-discrete-mathematics} having a runtime complexity of $\mathcal{O}(n^3)$, where $n$ is the size of the graph, or—in this case—the side length of the \ac{DBM} zone matrix. %, for evaluating a single successor.
When the variable order for two \acp{SC} is the same, this normal form is unique in the sense that two semantically equal \acp{SC} also have the same representation in the normalized form. This is useful since we can detect in the \ac{SC} graph when two paths with different firing histories end up in the same \ac{SC}. Thus, an \ac{SC} graph is, similarly to a marking graph, often finite and can therefore be completely analyzed.

Although it is possible to store the density function $f_\tau()$ numerically, e.g., with the help of a matrix measuring the density in a grid-like manner, it is beneficial to deal with an exact analytical representations instead.
In this context, it is helpful to restrict the class of possible firing distribution times which are generally enough to cover a wide range of different distributions, but it it still possible to mechanically perform standard operations on them, e.g., integration.
One possible class is called \emph{expolynomial}, which is an extension of polynomials, and is defined as follows \cite{stochastic-state-classes,bernstein-expolynomials-1,bernstein-expolynomials-2}:
\begin{definition}[Expolynomial]
    An expolynomial is a sum of products of monomials with an exponential function, concisely expressed with the following sum expression with parameters $\alpha_i \in \mathbb{N}$, $\lambda_i \in \mathbb{R}$ with $i\in \{1, 2, ..., n\}$:
    \begin{align*}
        f(x) = \sum_{i=1}^{n} c_i x^{\alpha_i} e^{-\lambda_i} x
    \end{align*}
\end{definition}
Note that we restrict the domain of expolynomials when applied to \acp{SSC} with an additional \ac{DBM} zone as explained in Section~\ref{sec:non-deterministic-analysis}. Thus, for a domain $D$, we have to scale the expolynomial such that it represents a \ac{PDF}, or more technically, we have to calculate a scaling factor $c\in \mathbb{R}^+$ such that $\int_{x\in D} c \cdot f(x) = 1$.
This class of distributions covers a wide range of regularly used distributions, e.g., exponential, immediate, or deterministic distributions. Also, uniform distributions are supported since it holds $f(x) = \mathbb{1}_{[a,b]}(x) \cdot x^0$, so it is a polynomial with additional support restriction.
Under this assumption, we can set up an analytical representation for a region $R$ that covers all of our desired timings~\cite{bernstein-polynomials-1}:
\begin{definition}[Multivariate expolynomial]
    An expolynomial can easily be extended to multiple dimensions, using parameters $\alpha_{i,j} \in \mathbb{N}$, $\lambda_{i,j} \in \mathbb{R}$ with $i\in \{1, 2, ..., n\}$ and $j\in \{1, 2, ..., g\}$:
    \begin{align*}
	      f(x_1, ..., x_{g}) = \sum_{i=1}^{n} c_i \cdot \prod_{j=1}^{g} x_j^{\alpha_{i,j}} e^{-\lambda_{i,j} x_j}
    \end{align*}
\end{definition}

{\color{red}Explain that we can evaluate to be at an \ac{SSC} at a certain time $0$}

\subsection{Confidence Intervals for Regular Simulation}
This section discusses how the estimation of the transient reward probabilities are obtained and elaborates on the effect on the width of \acp{CI} when using the mixed analysis with \acp{SSC} and simulation in comparison to a regular \ac{MC} simulation. For mathematical analysis, we characterize the transient reward of the system at model time $t$ with the random variable $X$ having mean $\mu$. As the reward is either $1$ or $0$ depending on if the marking condition is fulfilled, the \ac{RV} $X$ is Bernoulli distributed. Thus, the variance of $X$ can be calculated with $\sigma_\emph{sim}^2 = \mu (1 - \mu)$ when knowing the mean $\mu$.
When resorting to regular simulation, we estimate $\mu$ by calculating
\begin{align}
    \overline{X}_\emph{sim} = \frac{\sum_{i=1}^{n}x_i}{n}\text{,}
    \label{eq:standard-estimator-sim}
\end{align}
where $x_i$ is a sample from $X$ for $i\in \{1, 2, ..., n\}$.
Under the assumption that $n$ is chosen large enough, we know that $\overline{X}_\emph{sim}$ converges to:
\begin{align}
    \overline{X}_\emph{sim} \rightarrow \mathcal{N} \left(\mu, \frac{\sigma_\emph{sim}^2}{n}\right) \quad \iff \quad \frac{\overline{X}_\emph{sim} - \mu}{\sigma_\emph{sim} / \sqrt{n}} \rightarrow \mathcal{N}(0, 1)
    \label{eq:convergence_sim_normal}
\end{align}
We can rearrange Equation~\ref{eq:convergence_sim_normal} and determine the \ac{CI} for $\mu$ with
\begin{align}
    \left[\overline{X}_\emph{sim} - z_{\alpha/2}\cdot\frac{\sigma_\emph{sim}}{\sqrt{n}}, \overline{X}_\emph{sim} + z_{\alpha/2}\cdot\frac{\sigma_\emph{sim}}{\sqrt{n}}\right]\text{,}
\end{align}
where $z_{\alpha/2}$ corresponds to the $\alpha/2$-quantile for the standard normal distribution and $\sigma_\emph{sim}^2$ can be estimated with $\Tilde{\sigma}_\emph{sim}^2 = \overline{X}(1 - \overline{X})$.

{\color{red}Also explain that there are other estimators, e.g., Wilson's score interval which work better for a small sample size and low mean}

... the Wilson score interval~\cite{TODO}, which can be calculated with:
\begin{align*}
    \left[\frac{\overline{X} + \frac{z_{\alpha/2}}{2n} - z_{\alpha/2}\sqrt{\frac{\overline{X}(1 - \overline{X})}{n} + \frac{z_{\alpha/2}}{4n^2}}}{1 + \frac{z_{\alpha/2}}{n}}, \frac{\overline{X} + \frac{z_{\alpha/2}}{2n} + z_{\alpha/2}\sqrt{\frac{\overline{X}(1 - \overline{X})}{n} + \frac{z_{\alpha/2}}{4n^2}}}{1 + \frac{z_{\alpha/2}}{n}}\right]
\end{align*}

% \subsection{Connection between Stochastic State Classes and Simulation}
% \label{sec:dualism-ssc-simulation}

% Next, we elaborate on the connection between \acp{SSC} and discrete event simulation.
% In principle, \acp{SSC} only summarize all possible transitions from one state to another under the observation of all possible timing configurations. By running simulations, we implicitly sample after each firing step a point from an \ac{SSC}.
% The \acp{SSC} create a possibly infinitely large graph that characterizes the firing times of the transitions in a certain state.
% When handling the \acp{SSC} and the transitions as a tree without loops, e.g., not combining different firing histories that lead up in the same \ac{SSC}, we can characterize each \ac{SSC} by its firing history. This allows us to determine in which \ac{SSC} a simulation offspring currently is.
% \begin{figure}
%     \centering
%     \includegraphics{gfx/fig_dualism_ssc_simulation.pdf}
%     \caption{Connection between \acp{SSC} and simulation}
%     \label{fig:ssc_simulation_dualism}
% \end{figure}
% This idea is illustrated in Figure~\ref{fig:ssc_simulation_dualism}. If we sample any point out of the initial \ac{SSC} using its respective distribution, we can conduct the simulation until we reach the successor \ac{SSC}. The successor \ac{SSC} out of an initial \ac{SSC} can be determined by evaluating which transition will be fired first.
% By repeating this procedure multiple times and collecting the simulation points in one \ac{SSC}, we get an approximation of the resulting \ac{SSC}.
% Furthermore, we can conduct a mixture of \ac{SSC} and simulation, if we condition an \ac{SSC} and only evolve this part.
% Although this idea is theoretically achievable, it is unclear if it has practical benefits, since we introduce uncertainties by not fully analyzing the \ac{SSC}, but still have to rely on the expensive calculations with \acp{SSC}. Thus, it was not realized in the developed prototype and remains future work.
% Apart from that, it is worth mentioning that a single simulation instance can be seen as an \ac{SSC} without stochastic uncertainties. Thus, we can also expand \acp{SSC} from a discrete point in time. This approach will be analyzed in detail in Section~\ref{sec:resume-ssc}.


==> 99-old-previous-knowledge.tex <==
\begin{comment}
\section{Incorporating Knowledge from Simpler Representation}
\label{sec:knowledge-simpler-repres}

% We can employ \acp{SC} to analyze all reachable states under consideration of timing constraints using \acp{SC} and incorporate probabilities with \acp{SSC}.
As previously mentioned, the runtime of creating the \ac{SC} analysis graph is usually much smaller than for \acp{SSC}. Thus, there exists many models where the analysis with \ac{SC} is feasible, while for \acp{SSC} it is not. We can make use of this property by gaining information of the model to decide when to employ \acp{SC} and when \acp{SSC}. This approach is motivated by research around the automatic application of \ac{I-SPLIT} techniques which are built upon estimating the importance of a state using alternative methods~\cite{carlos-budde}.

\begin{figure}
    \centering
    \includegraphics{gfx/fig_idea_strategy.pdf}
    \caption{Illustration of the developed strategy}
    \label{fig:idea_strategy}
\end{figure}
We describe under a \emph{strategy} the guidelines for deciding when to do an expansion with \ac{SSC} and when to switch to simulation instead. The core idea of the proposed strategy is given in Figure~\ref{fig:idea_strategy} and it proposes to do an expansion for an \ac{SSC} $\Sigma$ when at least on of the following properties is fulfilled:
\begin{enumerate}
    \item The maximum number of firings for reaching an \ac{SSC} is smaller or equals than a threshold \emph{max\_dist\_root}.
    \item When an \ac{SSC} lies on a direct path according to the previous \ac{SC} analysis (meaning that its minimum distance to the target decreases by one), it is analyzed analytically.
    \item The distance to the target of an \ac{SSC} $\Sigma$ is smaller or equals to \emph{max\_dist\_target}, when there was at maximum deviation of \emph{max\_offset} to the target.
\end{enumerate}

\textcolor{red}{Heuristic with offsets: Strategy (either near enough the beginning or maximum deviation from shortest distance)}

\textcolor{red}{Gaining information through simpler \ac{SSC} graph}

\textcolor{red}{E.g., State Class Graph}
\end{comment}

